Digraph Signal Processing with Generalized Boundary Conditions

Signal processing on directed graphs (digraphs) is problematic, since the graph shift, and thus associated filters, are in general not diagonalizable. Furthermore, the Fourier transform in this case is now obtained from the Jordan decomposition, which may not be computable at all for large graphs. We propose a novel and general solution for this problem based on matrix perturbation theory: We design an algorithm that adds a small number of edges to a given digraph to destroy nontrivial Jordan blocks. The obtained digraph is then diagonalizable and yields, as we show, an approximate eigenbasis and Fourier transform for the original digraph. We explain why and how this construction can be viewed as generalized form of boundary conditions, a common practice in signal processing. Our experiments with random and real world graphs show that we can scale to graphs with a few thousands nodes, and obtain Fourier transforms that are close to orthogonal while still diagonalizing an intuitive notion of convolution. Our method works with adjacency and Laplacian shift and can be used as preprocessing step to enable further processing as we show with a prototypical Wiener filter application.

==> Counterexamples.tex <==

In this appendix we list (counter)examples to properties of directed
graphs and the proposed edge adding algorithm, which we wondered if
they hold.


\mypar{Strong connectedness} There is no connection between strong
connectedness, i.e. every nodes is reachable from each other node, and
diagonalizabilty or invertibility of the adjacency matrix. Indeed
after adding the first edge to the directed grid in
Fig.~\ref{fig:DirectedGrid} the graph is strongly connected but has a
non-trivial Jordan block to the eigenvalue $0$, turning it into a
non-diagonalizable, non-invertible graph.


\mypar{Jordan block eigenvalues} Every number, which is an eigenvalue
of a directed graph, can appear as eigenvalue with non-trivial Jordan
structure of the adjacency matrix. Indeed take any such graph $G$ and
choose any nodes as root. The rooted product with the directed path
graph is obtained by identifying the root of a copy of $G$ with each
vertex of the path graph. The rooted product graph has then a Jordan
block to each eigenvalue of $G$ with size the size of the path graph.


\mypar{Diagonalizabilty of $A$ and $L$} Neither diagonalizability of
the adjacency matrix $A$ implies diagonalizability of the directed
Laplacian $L = D - A$ nor the either way around. Indeed in
Fig.~\ref{fig:CounterexampleDiagonalizability} we show counterexamples
for each direction.
\begin{figure}
    \centering
    \subfloat[\label{subfig:AdjacencyNonDiag}]{
      \includegraphics[width=0.25\linewidth]{BadEdgeExample}
    }
    \hspace{2em}
    \subfloat[\label{subfig:LaplacianNonDiag}]{
      \includegraphics[width=0.27\linewidth]{NonDiagLaplacianButAdjacency}
    }
    \caption{A digraph (a) which has a diagonalizable directed Laplacian
      but a non-diagonalizable adjacency matrix. And a digraph (b) which
      has a diagonalizable adjacency matrix but a non-diagonalizable
      directed Laplacian.}
    \label{fig:CounterexampleDiagonalizability}
\end{figure}


\mypar{One edge is not enough} One can in general not destroy Jordan
blocks to different eigenvalues at once. A counter example is shown in
Fig.~\ref{fig:NotOneEdgeFixableDigraph}. The conditions for destroying
the blocks are $b_{3,1}\neq 0$ and $b_{6,1} + b_{6,4}\neq 0$, which
cannot be satisfied with one edge. However note that choosing
$b_{6,1}$ reduces the size of the other block from three to two.

% Figure: Counterexample: Cannot destroy two birds with one stone
% ---------------------------------------------------------------
\begin{figure}\centering
\subfloat[\label{subfig:NotOneEdgeFixableGraph}]{
	\includegraphics[width=0.25\linewidth]{NotOneEdgeFixableDigraphPPT}
      }\
      
\subfloat[\label{subfig:NotOneEdgeFixableAdjacency}]{
  $
  \begin{bsmallmatrix}
      0& 1& 0& 1& 0& 0\\ 
      0& 0& 1& 0& 0& 0\\ 
      0& 0& 0& 0& 0& 0\\ 
      0& 0& 0& 1& 1& 0\\ 
      0& 0& 0& 0& 1& 1\\ 
      0& 0& 0& 0& 0& 1
  \end{bsmallmatrix}$
}
    \hspace{0.5em}
\subfloat[\label{subfig:NotOneEdgeFixableJordan}]{
  $
  \begin{bsmallmatrix}
      0 & 1 & 0 \\
      0 & 0 & 1 \\
      0 & 0 & 0 \\
      & & & 1 & 1 & 0\\
      & & & 0 & 1 & 1 \\
      & & & 0 & 0 & 1
  \end{bsmallmatrix}$
}
\caption{A digraph (a) with adjacency matrix in (b) and JNF (c). The two blocks cannot be destroyed with one edge only.}\label{fig:NotOneEdgeFixableDigraph}
\end{figure}

%Consider the graph in Fig.~\ref{fig:NotOneEdgeFixableDigraph}.
%The corresponding eigenvectors of the Jordan blocks are
%\begin{equation}
%    \label{eq:EigenvectorsNotOneEdgeFixableDigraph}
%    u_0 =
%    \begin{bsmallmatrix}
%        0 \\
%        0 \\
%        1 \\
%        0 \\
%        0 \\
%        0 
%    \end{bsmallmatrix},
%    v_0 =
%    \begin{bsmallmatrix}
%        1 \\
%        0 \\
%        0 \\
%        0 \\
%        0 \\
%        0            
%    \end{bsmallmatrix},
%    u_1 =
%    \begin{bsmallmatrix}
%        0 \\
%        0 \\
%        0 \\
%        0 \\
%        0 \\
%        -1 
%    \end{bsmallmatrix},
%    v_1 =
%    \begin{bsmallmatrix}
%        -1 \\
%        0 \\
%        0 \\
%        -1 \\
%        0 \\
%        0
%    \end{bsmallmatrix}
%\end{equation}


\mypar{Adding edge yielding non-invertibility} The destruction of
Jordan blocks can introduce new $0$ eigenvalues, as shown in
Fig.~\ref{fig:NewEdgeNoninvertible}, which then requires additional
steps for their destruction.
\begin{figure}
    \centering
    \subfloat[\label{subfig:NewEdgeNoninvertible}]{
      \includegraphics[width=0.45\linewidth]{NewEdgeNoninvertible}
    }\
    
    \subfloat[\label{subfig:NewEdgeNoninvertibleBefore}]{
      $\begin{bsmallmatrix}
          1 & 1 \\ 
          0 & 1  \\ 
          & & \omega_3^2 & 1 \\ 
          & & 0 & \omega_3^2  \\ 
          & & & & \omega_3 & 1 \\ 
          & & & & 0 & \omega_3  \\ 
      \end{bsmallmatrix}$
    }
    \hspace{0.5em}
    \subfloat[\label{subfig:NewEdgeNoninvertibleAfter}]{
      $\begin{bsmallmatrix}
          & 0 & 1 & 0\\ 
          & 0 & 0 & 1 \\ 
          & 0 & 0 & 0 \\ 
          & & & & 2^{1/3} \\  
          & & & & & -(-2)^{1/3} \\
          & & &  &  &  & (-1)^{2/3} 2^{1/3} \\
      \end{bsmallmatrix}$
    }    
    \caption{A graph where the introduction of a new edge makes
      the adjacency matrix non-invertible. In (b) the
      Jordan normal form before and in (c) after adding the edge is
      shown.}
    \label{fig:NewEdgeNoninvertible}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


